An empirical study on the names of points of interest and their changes with geographic distance

While Points Of Interest (POIs), such as restaurants, hotels, and barber shops, are part of urban areas irrespective of their specific locations, the names of these POIs often reveal valuable information related to local culture, landmarks, influential families, figures, events, and so on. Place names have long been studied by geographers, e.g., to understand their origins and relations to family names. However, there is a lack of large-scale empirical studies that examine the localness of place names and their changes with geographic distance. In addition to enhancing our understanding of the coherence of geographic regions, such empirical studies are also significant for geographic information retrieval where they can inform computational models and improve the accuracy of place name disambiguation. In this work, we conduct an empirical study based on 112,071 POIs in seven US metropolitan areas extracted from an open Yelp dataset. We propose to adopt term frequency and inverse document frequency in geographic contexts to identify local terms used in POI names and to analyze their usages across different POI types. Our results show an uneven usage of local terms across POI types, which is highly consistent among different geographic regions. We also examine the decaying effect of POI name similarity with the increase of distance among POIs. While our analysis focuses on urban POI names, the presented methods can be generalized to other place types as well, such as mountain peaks and streets.

==> method.tex <==
%\vspace*{-0.4cm}
\section{Methods}
%\vspace*{-0.2cm}

In this work, we investigate the \textit{localness} of POI names. The similarity examined here is \textit{collective similarity}, namely how the names of POIs in one geographic region are similar or dissimilar with those in another region. In other words, we are interested in the overall naming style difference across geographic regions, instead of how individual POI names differ from each other. 

Multiple methods exist that can be employed for measuring the collective similarity of the names of POIs in different regions. In this work, we experiment with 3 different models, which are count-based vector, term frequency and inverse document frequency (TF-IDF), and neural network embedding. All three methods are based on the idea of representing each geographic region as a vector based on the terms used in these areas, but they differ in the ways of deriving the values of the vectors. In the following, we describe their methodological details.

%Let $r_1$ and $r_2$ represent two geographic regions; let two sets, $\{ o_{11}, o_{12}, \dots , o_{1n}\}$ and $\{o_{21},  o_{22}, \dots , o_{2m}\}$, be the names of the POIs located in $r_1$ and $r_2$ respectively. 

%in different geographic regions from one perspective, namely how the naming of POIs changes over geographic distance. Intuitively, a strong \textit{localness }should lead to a strong negative relation between the distance of two regions and the similarity of POI names in these regions. While it is expected that POI names should show, at least, some localness, this study examines whether there exists a strong and statistically significant relation between POI naming and geographic distance.

Let $r_1$ and $r_2$ represent two geographic regions, and each region contains a set of POIs. In a count-based vector approach, we derive the vector for a geographic region by simply counting the frequencies of words used in the POI names of this region. A common vocabulary $V$ can be constructed based on all the words of the POI names in a dataset. Thus, the names of POIs in the two regions, $r_1$ and $r_2$, can be collectively represented as two vectors:
\begin{eqnarray}
 <{\ w}_{11},\ {\ w}_{12},\ \dots ,\ {\ w}_{1\left|V\right|}> \\
 <{\ w}_{21},\ {\ w}_{22},\ \dots ,\ {\ w}_{2\left|V\right|}>
\end{eqnarray}
%\[\ <{\ w}_{11},\ {\ w}_{12},\ \dots ,\ {\ w}_{1\left|V\right|}>\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ (1)\] 
%\[\ <{\ w}_{21},\ {\ w}_{22},\ \dots ,\ {\ w}_{2\left|V\right|}>\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ (2)\] 
where $\left|V\right|$ represents the size of the vocabulary, and ${\ w}_{ij}$ represents the count of word $j$ in the POI names in geographic region $i$. All vectors  for different regions are in the same dimension $|V|$.

While the count-based vector considers only the frequency of words, TF-IDF captures the comparative differences of word usage in different geographic areas. Using TF-IDF, the value of each vector, $w_{ij}$, is calculated as Equation \ref{tf-idf}:
\begin{equation}
w_{ij} = \mathit{tf}_{ij} \times (\log\frac{|N|}{|G_j|} +1 ) \label{tf-idf}
\end{equation}
where $\mathit{tf}_{ij}$ is the term frequency of word $j$ in  geographic region $i$, $|N|$ is the total number of geographic regions in the dataset, and $|G_j|$ is the number of regions that contain the word $j$. The count-based vector approach can be considered as a simple version of TF-IDF in which IDF is not considered. TF-IDF emphasizes the words that appear frequently in a local region but not frequently in other areas.  
 


%\[S=\ \frac{\sum^{|V|}_{j=1}{w_{1j}w_{2j}}}{\sqrt{\sum^{|V|}_{j=1}{w^2_{1j}}}\ \sqrt{\sum^{|V|}_{j=1}{w^2_{2j}}}}\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ (3)\] 
While the count-based vector and TF-IDF are descriptive approaches, the third model, neural network embedding, is a predictive approach. Specifically, we employ \textit{Word2vec} \cite{mikolov2013distributed} to learn \textit{embeddings} for different geographic regions based on the names of the POI located in these areas. The skip-gram architecture of word2vec is utilized, which learns embeddings by predicting the words of POI names based on the given geographic region (i.e., what words are likely to be used for POI names if the geographic region is \textit{Phoenix, AZ}). The embeddings are condensed vectors, and the POI names in $r_1$ and $r_2$ can be represented as the two vectors below:
\begin{eqnarray}
<{\ u}_{11},\ {\ u}_{12},\ \dots ,\ {\ u}_{1\left|d\right|}> \\
<{\ u}_{21},\ {\ u}_{22},\ \dots ,\ {\ u}_{2\left|d\right|}>
\end{eqnarray}
%\[<{\ u}_{11},\ {\ u}_{12},\ \dots ,\ {\ u}_{1\left|d\right|}>\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ (4)\] 
%\[<{\ u}_{21},\ {\ u}_{22},\ \dots ,\ {\ u}_{2\left|d\right|}>\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ (5)\] 
where $d$ is the dimensionality of the embeddings, which can be decided empirically and which are usually much smaller than the size of the vocabulary $|V|$. $u_{ij}$ is a value learned from the POI dataset using a neural network model, which aims to minimize the objective function in Equation \ref{negativesampling}:
\begin{equation}
J\boldsymbol{=\ }-\ {\mathrm{log} \sigma \left({\boldsymbol{w}}^T_o\boldsymbol{r}\right)\ }-\ \sum^K_{k=1}{{\mathrm{log} \sigma \left(-{\boldsymbol{w}}^T_k\boldsymbol{r}\right)\ }} \label{negativesampling}
\end{equation} 
%\[J\boldsymbol{=\ }-\ {\mathrm{log} \sigma \left({\boldsymbol{w}}^T_o\boldsymbol{r}\right)\ }-\ \sum^K_{k=1}{{\mathrm{log} \sigma \left(-{\boldsymbol{w}}^T_k\boldsymbol{r}\right)\ }}\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ (6)\] 
where $\boldsymbol{r}$ is the embedding of one geographic region, ${\boldsymbol{w}}_o$ is the embedding of a word that is indeed used for the POI names in region $\boldsymbol{r}$, while ${\boldsymbol{w}}_k$ is the embedding of a word not used in region $\boldsymbol{r}$. $\sigma $ is a sigmoid function: $\sigma \left(x\right)=\ \frac{1}{1+\ e^{-x}}$.

% as defined in Equation \ref{sigmoid}:
%\begin{equation}
%\sigma \left(x\right)=\ \frac{1}{1+\ e^{-x}}  \label{sigmoid}
%\end{equation} 
%\[\sigma \left(x\right)=\ \frac{1}{1+\ e^{-x}}\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ (7)\] 
%With the embeddings learned for different regions based on the POI names there, we can use cosine similarity again to measure the collective similarity of the POI names in different regions. 


In all three methods, different geographic regions are represented as vectors in the same dimension. Thus, cosine similarity can be employed to measure the similarity of any two vectors (Equation \ref{cosine}). The similarity value, $S$, is then used as the collective similarity between the POI names in two regions.
\begin{equation}
S =\ \frac{\sum^{d}_{j=1}{w_{1j}w_{2j}}}{\sqrt{\sum^{d}_{j=1}{w^2_{1j}}}\ \sqrt{\sum^{d}_{j=1}{w^2_{2j}}}} \label{cosine}
\end{equation} 

